Towards Computationally Verifiable Semantic Grounding for Language Models

The paper presents an approach to semantic grounding of language models (LMs) that conceptualizes the LM as a conditional model generating text given a desired semantic message formalized as a set of entity-relationship triples. It embeds the LM in an auto-encoder by feeding its output to a semantic parser whose output is in the same representation domain as the input message. Compared to a baseline that generates text using greedy search, we demonstrate two techniques that improve the fluency and semantic accuracy of the generated text: The first technique samples multiple candidate text sequences from which the semantic parser chooses. The second trains the language model while keeping the semantic parser frozen to improve the semantic accuracy of the auto-encoder. We carry out experiments on the English WebNLG 3.0 data set, using BLEU to measure the fluency of generated text and standard parsing metrics to measure semantic accuracy. We show that our proposed approaches significantly improve on the greedy search baseline. Human evaluation corroborates the results of the automatic evaluation experiments.

==> Peirce_ Semantically Grounded LMs/dataset.tex <==
\section{Data Set}

The WebNLG corpus~\cite{gardent-etal-2017-creating} comprises of sets of triplets describing facts (entities and relations between them) and the corresponding facts rendered in form of natural language text. The corpus contains sets of up to 7 triplets alongside one or more reference texts for each set. As explained in Section 2 of~\citep{castro-ferreira-etal-2020}, the English dev set consists of categories and entities seen in the training data; the English test set (D2T) consists of a mixture of seen entities and categories, as well as unseen entities and 5 unseen categories (28\%, 22\% and 50\%, respectively), making it hard to expect correct text generation and/or semantic parsing from our models. Nevertheless, we experiment in this condition as well.

The dataset can be used for work in both natural language generation and the reverse task of triplets extraction. Its main use was for the WebNLG natural language generation challenge with the goal to map the sets of triplets to text, including referring expression generation, aggregation, lexicalization, surface realization, and sentence segmentation. 

The initial (2017) WebNLG shared task required participating systems to generate English text from a set of DBpedia triples~\cite{gardent-etal-2017-webnlg} whereas the more recent (2020) WebNLG 3.0 data set used for the WebNLG+ challenge~\citep{castro-ferreira-etal-2020} additionally includes generation into Russian and semantic parsing of English and Russian texts, encompassing four tasks: RDF-to-English, RDF-to-Russian, English-to-RDF and Russian-to-RDF.

We only use WebNLG 3.0 English data, starting from a pre-trained language model~\cite{raffel2019T5} and fine-tuning it on the WebNLG training data for either LM or semantic (RDF) parsing. Since the model uses a encoder-decoder architecture we feed the conditioning information (RDF triples when incrementally training the LM or natural language text when training the SP) to the encoder and then let the decoder generate the output sequence (natural language text or RDF triples, respectively). We note that the exact order of the RDF triples for a given reference text is a degree of freedom that we could experiment with.

==> Peirce_ Semantically Grounded LMs/model.tex <==
\section{Model}

%\cc{We need to reconcile the notation here with that in the Intro}

Let $W$ be a text unit (a sentence in the WebNLG data) and $S$ be a representation of the semantic message of $W$ (a sequence of WebNLG triples). We define a semantic LM and a semantic parser as two sequence-to-sequence models:
\begin{itemize}
    \item $P(W|S;\theta)$: a \textit{semantic LM} trained to encode a semantic message $S$ into text units $W$;
    \item $R(S|W;\phi)$: a \textit{semantic parser (SP)}, trained to decode the semantic message $S$ from a text unit $W$.
\end{itemize}
Our objective is to develop a method that generates computationally verifiable text: given a semantic message $S^*$, we would like to find a verbalization $W^*$ such that running the semantic parser $R$ on $W^*$ will result in a semantic message $S^+$ as close as possible to the original $S^*$. In this work we compare a baseline to two methods designed to achieve this objective:  a sampling approach and a new approach we refer to as ``greedy finetuning''.

In the baseline approach we decode greedily with $P(W|S;\theta)$ to encode the input semantic message $S^*$ into the text unit $W^*$. In the sampling approach, we sample text units from the $P(W|S=S^*; \theta)$ model using temperature or nucleus sampling \cite{holtzman2019curious}, then run the semantic parser on every sampled text unit, finally select as $W^*$ the text unit that maximizes the $F1$ score between the semantic parse $S^+ = \argmax_{s} R(S|W^*;\phi)$ and the input semantic message $S^*$. 

In ``greedy finetuning'' we take a more complex approach and re-estimate the LM based on feedback from the semantic parser. We iteratively perform greedy decoding  with the semantic LM $P$ to obtain a text unit $W_i$, then adjust the semantic LM $P$ while keeping the SP model $R$ ``frozen'' in order to increase the probability of reconstruction of the correct semantic message. After $k$ steps, we pick the final text unit $W^*$ from the set $\{W_1, \ldots, W_k\}$, choosing the one that leads to the best F1 score between the decoded semantic message $S^+$ and the original message $S^*$.

The semantic LM update in ``greedy finetuning'' is performed by taking a gradient ascent step on the following objective function:
\begin{align*}
  J(S^*, S^+; \theta, \phi) = \E_{W \sim P(\cdot|S^*;\theta)} [R(S^+|W;\phi)],
  \label{eq:obj}
\end{align*}
where keeping the semantic parser frozen corresponds to keeping $\phi$ constant and only updating $\theta$.\footnote{We note that greedy finetuning is expensive since it requires updating all the parameters of the semantic LM $k$ times for every inference batch. The approach could be made substantially more efficient, however, by employing parameter efficient methods such as prompt tuning \cite{lester2021power}.}

Since both $P$ and $R$ are neural networks, the gradient ascent step for $\phi$ can \textit{mostly} be computed by backpropagation. However, the objective $J$ is not differentiable because it requires auto-regressively decoding from the model $P$ to sample values for $W$ and estimate the expectation of correct reconstruction. We get around this difficulty by sampling the text unit $W$ using greedy decoding and then employing the straight-through gradient estimator (\newcite{bengio2013estimating}, \newcite{hinton2012neural}). The estimator is illustrated in more detail in section \ref{sec:st-approx}.

In addition to (1) greedy (baseline), (2) sampling and (3) greedy finetuning, we consider two ensemble methods: (4) greedy+sampling and (5) greedy finetuning+sampling. Greedy+sampling will run both methods (1) and (2), and then pick the verbalization $W^*$ that leads to the reconstruction with the highest F1 score. Greedy finetuning+sampling will similarly pick the best output after running methods (2) and (3).

% CA: This could be future work.
% Another observation is that although we use $s$ as the target sequence for the SP model, in fact any permutation of the E-R triples in $s$ would be an equally good target for the SP model. A two step estimation algorithm that chooses the target semantic parse $s*$ by evaluating all permutations $\pi(s)$ for the input semantic parse $s$ under the $R(S|w*;\phi)$ model and picks the most likely one before the back-propagation step is also possible.

\subsection{Straight Through Approximation}
\label{sec:st-approx}
To propagate the gradient of $J$ through the SP into the language model we need to compute
\begin{equation*}
    \frac{\partial R(S|W^*;\phi)}{\partial \theta},
\end{equation*} 
where $W^* = \argmax P(W|S^+; \theta)$ is computed using greedy search $\textsc{g\_search}$.

Following \newcite{hinton2012neural}, during the forward pass we transmit the text tokens $W^*$, and during the backward pass we pretend as if for every token the real value distribution over the vocabulary was transmitted instead. For this purpose, we can regard the $W^*$ sequence passed to the SP as a binary tensor  
\begin{equation*}
W^* = \textsc{one\_hot}(\textsc{g\_search}(\log P(W|S^+; \theta)))
\end{equation*} 
of shape $(b, l, v)$ where $b$ is the batch size, $l$ is the maximum length in tokens or word-pieces for text sequences including padding, and $v$ is the size of the vocabulary. 
	
In the straight-through (ST) approximation with automatic differentiation, we replace the $W^*$ tensor in the computational graph with the following:
\begin{eqnarray*}
W^*_\mathrm{ST} &= & P(W^*|S^+; \theta) +\\
& & \mathrm{S\_G}[W^* - P(W^*|S^+; \theta)]
\end{eqnarray*}
where the $\mathrm{S\_G}[\cdot]$ stop-gradient operator is the familiar pass-through in the forward direction and none-shall-pass in back-propagation. Thus in the forward direction the computation will proceed with $W^*_\mathrm{ST} = W^*$, however in the backward direction the computation will behave as if $W^*_\mathrm{ST} = P(W^*|S^+; \theta)$.
%\cc{Is this what you implemeneted Chris? There's also the option of masking the logP tensor with the one-hot mask.}

% CA: This would also be future work.
% If we want an ST approximation for the case where instead of greedy search we use sampling we need a way to mix the probability tensors for each of the sampled hypotheses $w_1(s), ..., w_K(s)$. A simple possibility is to weigh the $P()$ multinomial distribution over $v$ for each hypothesis $w_k(s)$ at a given time step $t$ by the prefix probability of the hypothesis up to that point, and re-normalize them to 1.0:
% $$w_k(t) = P(w_k(s)[0:t-1]) / sum_k P(w_k(s)[0:t-1])$$

% More in detail, we can express the expectation in equation \ref{eq:obj} as
% \begin{align}
%   J(s; \theta, \phi) = \sum_w P(w|s;\theta) R(s|w;\phi)
% \end{align}
% and its gradient with respect to $\theta$
% \begin{align}
%   \hat{\frac{\partial J}{\partial \theta}} = 
  
% \end{align}


% assume we obtain a sample textual generation $\hat{w}$ for a given semantic message $s$ from $P(W|s;\theta)$ either with temperature sampling or greedy decoding. We approximate the expectation in equation \ref{eq:obj} with the $J(s; \theta, $


==> Peirce_ Semantically Grounded LMs/related_work.tex <==
\section{Related Work}

The idea of building auto-encoders for language where the latent variable itself is language was previously explored by \newcite{miao2016language}, where the authors propose an inference approach for sentence compression based on variational auto-encoders. Unlike  \newcite{miao2016language}, our work draws the latent representation from a probability distribution conditioned on the input semantic parse, rather than a background language model. The optimization strategy is also different since we perform a small number of gradient descent steps instead of employing variational inference.

\newcite{sun-etal-2018-logician} tackle a very similar problem in a reinforcement learning setup, training both LM ("narrator") and open information extraction models jointly. Our work fixes the semantic parser while still taking advantage of the ability to back-propagate the error of reconstructing the correct semantic message.

The approach of data-to-text-to-data is also a somewhat common evaluation strategy. Starting with \citet{wiseman2017challenges}, people have been using information extraction to match information in text with that of the input. More recent work like \citet{manning2021referenceless} tries to parse text into AMRs. In this work we go a step further and attempt to directly improve generation quality by sampling or by backpropagating parsing signals into the generation component.


==> Peirce_ Semantically Grounded LMs/results.tex <==
\definecolor{Gray}{gray}{0.9}

\section{Experiments}


\begin{table*}[t]
    \centering
    \begin{tabular}{l|ccccc} 
       Method                  & BLEU & METEOR & chrF++ & Triple P / R / F1 & Improved\\
       \hline
       greedy (baseline)                  & 0.64 &   0.46 &  0.76 & 0.93 / 0.87 / 0.90 & - \\
       \rowcolor{Gray}
       sampling                & 0.51 &   0.43 &  0.71 & 0.97 / 0.92 / 0.95 & - \\
       sampling (t=0.3, p=0.95) & 0.63 & 0.46  &  0.76 & 0.96 / 0.91 / 0.94 & - \\
       \rowcolor{Gray} greedy+sampling       & 0.60 &   0.46 &  0.75 & 0.98 / 0.93 / 0.95 & 0.20 \\
       greedy+sampling (t=0.3, p=0.95) & 0.63 & 0.47  &  0.76 & 0.96 / 0.91 / 0.94 & 0.14 \\
       \rowcolor{Gray}
       greedy finetuned & 0.62 &   0.46 &  0.76 & 0.96 / 0.91 / 0.93 & 0.13\\
       greedy f.+sampl. (t=0.3, p=0.95) & 0.63 & 0.46 & 0.76 & \textbf{0.97 / 0.92 / 0.95} & \textbf{0.17} \\
    \end{tabular}
    \caption{Automatic evaluation of our method on ``seen'' test data (dev split of English WebNLG 3.0). Grayed rows have BLEU scores more than 1\% below the baseline. The ``Improved'' column displays the ratio of generations with a higher triple F1 compared to the greedy baseline.}
    \label{tab:automatic_eval_dev}
\end{table*}


\begin{table*}[t]
    \centering
    \begin{tabular}{l|ccccc} 
       Method                  & BLEU & METEOR & chrF++ & Triple P / R / F1 & Improved \\
       \hline
       Amazon AI (2020 1st)    & 0.54  & 0.42 &  0.69 &  \\
       bT5                     &  0.52 & 0.41 & 0.68 &  \\
       \hline
       greedy (baseline)                 & 0.54 & 0.41  &  0.69 & 0.58 / 0.50 / 0.54 & - \\
       \rowcolor{Gray}
       sampling                & 0.44 & 0.39  &  0.64 & 0.66 / 0.58 / 0.62 & - \\
       sampling (t=0.3, p=0.95) & 0.53 & 0.41  &  0.68 & 0.65 / 0.57 / 0.60 & - \\
       \rowcolor{Gray} greedy+sampling         & 0.51 & 0.41  &  0.67 & 0.67 / 0.59 / 0.63 & 0.31 \\
       greedy+sampling (t=0.3, p=0.95) & 0.54 & 0.41  &  0.69 & 0.65 / 0.57 / 0.61 & 0.23 \\
       greedy finetuned & 0.53 & 0.41  &  0.68 & 0.65 / 0.57 / 0.61 & 0.20 \\
       greedy f.+sampl. (t=0.3, p=0.95) & 0.53 & 0.41 & 0.68 & \textbf{0.69 / 0.61 / 0.65} & \textbf{0.34} \\
    \end{tabular}
    \caption{Automatic evaluation of our method on ``mixed: seen and unseen'' test data (test split of English WebNLG 3.0). Grayed rows have BLEU scores more than 1\% below the baseline. The ``Improved'' column displays the ratio of generations with a higher triple F1 compared to the greedy baseline.}
    \label{tab:automatic_eval}
\end{table*}

%\begin{table*}[t]
%    \centering
%    \begin{tabular}{l|ccccccc} 
%       \multicolumn{1}{c}{}& & & & \multicolumn{3}{c}{Triple}\\
%       Method                  & BLEU & METEOR & chrF++ &  P & R & F1 & Improved \\
%       \hline
%       bT5                                     & 0.52 & 0.68 & 0.68 & \\
%       \hline
%                       greedy (baseline)       & 0.47  & 0.36 & 0.65 & 0.87 & 0.83 & 0.85 & - \\
%       \rowcolor{Gray} sampling                & 0.40  & 0.35 & 0.62 & 0.93 & 0.91 & 0.92 & -\\
%       \rowcolor{Gray} greedy + sampling       & 0.44  & 0.36 & 0.65 & 0.94 & 0.92 & 0.93 & 0.31\\
%       \rowcolor{Gray} greedy finetuned.       & 0.45  & 0.36 & 0.64 & 0.92 & 0.90 & 0.91 & 0.23 \\
%       \rowcolor{Gray} greedy finetuned + sampling & 0.44 & 0.36 & 0.65 & 0.95 & 0.94 & 0.94 & 0.34 \\
%    \end{tabular}
%    \caption{Automatic evaluation of our method on the test split of Russian WebNLG. Grayed rows have BLEU scores more than 1\% below the baseline. \ca{Figure out why bt5 is better here!}}
%    \label{tab:automatic_eval_ru_test}
%\end{table*}


%\begin{table*}[t]
%    \centering
%    \begin{tabular}{l|ccccccc} 
%       \multicolumn{1}{c}{}& & & & \multicolumn{3}{c}{Triple}\\
%       Method                  & BLEU & METEOR & chrF++ &  P & R & F1 & Improved \\
%       \hline
%       greedy (baseline)                 & 0.35  &    0.32   &   0.58 & 0.76 & 0.69 & 0.72 & -\\
%       \rowcolor{Gray} sampling                & 0.29  &    0.30   &   0.56 & 0.85 & 0.80 & 0.82 & - \\
%       \rowcolor{Gray} greedy + sampling       & 0.32  &    0.31   &   0.58 & 0.87 & 0.82 & 0.84 & 0.40\\
%       greedy finetuned  & 0.35  &    0.32   &   0.58 & 0.86 & 0.80 & 0.83 & 0.31 \\
%       greedy finetuned + sampling & 0.34 & 0.32 & 0.58 & \textbf{0.90} & \textbf{0.85} & \textbf{0.87} & \textbf{0.44}\\
%    \end{tabular}
%    \caption{Automatic evaluation of our method on the dev split of Russian WebNLG. Grayed rows have BLEU scores more than 1\% below the baseline.}
%    \label{tab:automatic_eval_ru_dev}
%\end{table*}


\begin{table}
    \centering
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{l|ccc} 
       Model & F1 & P & R \\
       \hline
        Amazon AI (Shanghai) & 0.67 & 0.69 & 0.69 \\
        bt5 & 0.68 & 0.67 & 0.70 \\
        Our T5 & 0.63 & 0.63 & 0.64
    \end{tabular}}
    \caption{Exact match parsing performance of our T5 semantic parser (SP) on Text2RDF English WebNLG.
    }
    \label{table:parsing_acc}
\end{table}

% \begin{table}
%     \centering
%     \begin{tabular}{l|ccc} 
%       \multicolumn{1}{c}{}& \multicolumn{3}{c}{Triple} \\
%         &  P & R & F1 \\
%       \hline
%       dev   &   0.87 & 0.81 & 0.84 \\
%       test &   0.56 & 0.54 & 0.55 \\
%     \end{tabular}
%     \caption{Parsing performance of our T5 semantic parser (SP) on English WebNLG. \ca{TODO: Measure this with the official tool and compare to bt5.}}
%     \label{table:parsing_acc}
% \end{table}

%\begin{table}
%    \centering
%    \begin{tabular}{l|ccc} 
%       \multicolumn{1}{c}{}& \multicolumn{3}{c}{Triple} \\
%        &  P & R & F1 \\
%       \hline
%       dev   &   0.76 & 0.73 & 0.75 \\
%       test &   0.86 & 0.85 & 0.86 \\
%    \end{tabular}
%    \caption{Parsing performance of our T5 parsers on Russian WebNLG. \ca{TODO: Measure this with the official tool and compare to bt5.}}
%\end{table}

% We use the English data from \citet{castro-ferreira-etal-2020}. 
As semantic LM and semantic parser we train T5 XXL models on the training set split of WebNLG for 100 steps with a batch size of 256 examples. We then compare three main methods: (1) the greedy decoding baseline, (2) sampling with different temperatures and nucleus probability mass, (3) greedy finetuning. We additionally report ensembled of these methods. (1)+(2) is ``greedy+sampling'', where we perform both greedy decoding and sampling and then pick the generated text with highest semantic parsing F1 score. Similarly (2)+(3) is ``greedy finetuning+sampling''.

For the sampling approach we alway pick 4 samples, we set the temperature to either 1.0 or 0.3, and the nucleus probability mass to either 1.0 or 0.95. For the greedy finetuning approach we perform gradient descent steps  on $\theta$ with AdaFactor, with a learning rate of $10^{-3}$. We perform 4 iterations  and return the hypothesis with the best semantic reconstruction. Greedy finetuning is performed on batches of 64 examples.

% ChrisA: This is a good point. We will add this after pubapprove or after Arxiv submission.
% \sg{One thing you can expect in review is the question why beam search wasn't used which is pretty standard for the task setup and probably a stronger baseline.}

\subsection{Automatic Evaluation}

% Since our semantic parser is relatively far from perfect Recall (see Table~\ref{table:parsing_acc}) we cannot measure the extent to which generated text carries the desired semantics, or even a subset of it. Instead 
As an automatic metric of semantic grounding, we measure the standard Precision, Recall and F1 metrics used for evaluating semantic parsing accuracy, fixing the input WebNLG triples as reference and the triples reconstructed by the semantic parser as hypothesis. As for the fluency of the text generated by the LM, we measure it using BLEU \cite{papineni2002bleu}, METEOR \citep{banerjee2005meteor} and chrF++ \cite{popovic2017chrf++} against the human references in the D2T data sets. We note that there are between one and five references for each RDF triple, frequently two or three. 

The results of automatic evaluation on the English section of WebNLG 3.0 are shown in Tables \ref{tab:automatic_eval_dev} and \ref{tab:automatic_eval}. We first note that our greedy baseline matches the performance of the 2020 WebNLG winning system on BLEU and chrF++. Sampling and greedy finetuning increase triple F1 by 6\% and 7\% absolute on the test set, while keeping the BLEU score and other metrics within one point from the greedy baseline, showing that the semantic match with the desired input meaning can be significantly increased at minimal cost in the fluency of the generated text. The greedy finetuned+sampling ensemble gives us the highest performance, increasing triple F1 by 11\%, again keeping the fluency metrics within 1\% from the greedy baseline. The same overall trends can be observed for the WebNLG dev set in Table \ref{tab:automatic_eval_dev}. We additionally note that the sampling approach only performs well in this evaluation if temperature and nucleus probability mass are tuned.

We additionally report for both dev and test set the fraction of generations that with improved triple F1 compared to the greedy baseline. We only report the improved ratio for methods that are ensembled with greedy and so are guaranteed to always improve on automatically measured triple F1 compared to the baseline. We find that our best method, greedy finetuned+sampling, improves 34\% of our generations according to our automated metric of semantic verification.

As a sanity check for our semantic parser model, we report in Table \ref{table:parsing_acc} the performance of our T5 semantic parser on the official evaluation metrics of WebNLG Text2RDF. Since we only fine-tune T5 on the training split of WebNLG and we don't employ any additional techniques, the performance of our parser is competitive but lower than SotA systems.

% We report results for two setups: \textit{multitask} and \textit{no-multitask}. In both cases we initialize the LM parameters $\theta$ and the SP ones $\phi$ with the parameters of the T5 XXL model and then fine-tune on the training split of WebNLG. For the \textit{no-multitask} case, we fine-tune $\theta$ and $\phi$ separately on the parse-to-text and the text-to-parse tasks respectively. For the \textit{multitask} case, we tie $\theta$ and $\phi$ during fine-tuning on the training set, relying on an input prefix to tell the model whether it should perform the text generation (parse-to-text) or semantic parsing (text-to-parse) task. In either setup, we then freeze the parser parameters $\phi$ and only update the LM parameters $\theta$ while performing unsupervised optimization of the RDF triple reconstruction learning objective. We find that the \textit{no-multitask} setup performs substantially better in our experiments. \kg{This could be because the parsing and generation tasks perform best at a different number of epochs (for the no-multitask setting the parse-to-text task we stop at iteration number ?? and for the text-to-parse task we stop at iteration number ?? to optimize BLEU).}

\subsection{Human Evaluation}

\begin{table*}
    \centering
    \begin{tabular}{l|rrrrrr}
        Method             &  Examples &  Triples &  Fluency &  Precision &  Recall &  F-Score \\
        \hline
        reference         &     206   &   1278   &     1.00 &       0.77 &    0.91 &     0.84 \\
        \hline
        greedy (baseline) &     206   &   1278   & \bf 1.00 &       0.74 &    0.84 &     0.78 \\
        greedy + sampling &     115   &    719   &     0.99 &       0.74 &\bf 0.87 & \bf 0.80 \\
        greedy finetuned  &     112   &    675   &     0.98 &   \bf 0.76 &    0.84 & \bf 0.80 \\
    \end{tabular}
    \caption{Human evaluation results.  The row labeled ``reference'' has the evaluation of the human-generated reference text (provided as part of the test set).  Triples is the total number of triples rated, not the number of triples generated by the parser for a particular system. See text for details.}
    \label{tab:human_eval}
\end{table*}

Because our inference method relies on the SP, one could reasonably question whether it is appropriate to use the same SP also in the automatic evaluation. For example, it is possible that our method is learning to cheat by finding text with wrong semantics that the text-to-parse model incorrectly parses as the desired semantics.  In order to alleviate such concerns we augment the automatic evaluations with human ratings.

Ideally, expert annotators would encode the DBPedia semantics of reference text as well as system outputs. However, due to the size of DBPedia with tens of thousands of possible relations, it is infeasible for a human to perform the parsing task.  Instead, we present annotators with a text as well as candidate triples and ask them to evaluate whether each candidate triple is represented in the given text.  

We evaluate the text generated by our models in the following way: 
\begin{enumerate}
    \item Use the SP model to generate possible triples for the reference text as well as all model outputs. \label{step1}
    \item For the reference text and each system output, we present the raters with that text and the union of parse triples generated in step~\ref{step1}.
    \item For each triple, the raters verify whether it is implied by the text.
    \item We compute precision and recall for the reference text and each system with respect to the union of generated triples and the human ratings.
\end{enumerate}
We evaluate samples where the greedy decoding baseline did not produce the same result as greedy+sampling and greedy finetuned.  We see from Table~\ref{tab:automatic_eval_dev} that this happens in 23\% and 20\% of examples respectively.  We include the exact phrasing of the question as well as a screenshot of the rating interface in Appendix~\ref{sec:appendix_human_eval_template}.  In addition to the semantic annotation we also ask the raters to judge the fluency of the generated text. 

The results are shown in Table~\ref{tab:human_eval}.  The row labeled reference refers to the human-generated reference text which has a surprisingly low precision and recall.  The remaining rows have the same definitions as in Table~\ref{tab:automatic_eval_dev}.
% Recall that Table~\ref{tab:human_eval} is not a uniform sample over the development data, because we only evaluate examples where the prediction of greedy+sample or greedy finetuned is not the same as that of greedy decoding (20-23\% of examples).
We got 3-way annotations for 112 examples for greedy finetuned and 115 examples for greedy+sampling (and the corresponding 206 examples for greedy decoding).  Overall, we see that sampling improves recall while greedy finetuned improves precision, while not significantly changing the fluency of the text. Using bootstrap resampling on the examples, we find that greedy+sampling has significantly higher recall than greedy (p value 0.97), but greedy finetuned isn't better at the 95\% level in terms of precision (p value 0.948 with 10k samples).  The other metrics aren't significantly different.
% TODO: interannotator agreement

In addition to corroborating the results from automatic evaluation, the human eval show strikingly low precision and recall of the ``reference'' text.  We show two illustrative examples of losses.  First, we display an example below of a recall loss, where the annotator did not adhere strictly to the semantics.

\vspace{1em}
\hspace{-1em}\begin{tabular}{@{}|p{0.94\columnwidth}|@{}}
    \hline
    \textbf{Input:} \small\texttt{Zaoyang | isPartOf | Hubei}  \\
    \small\texttt{Nie\_Haisheng | birthPlace | Zaoyang}  \\
    \hline
    \textbf{Target:} Nie Haisheng is from Zaoyang in Hubei province.\\
    \hline
\end{tabular}
\vspace{1em}

In this example, the rater chose to realize the \texttt{birthPlace} relation using the phrase \emph{is from}, but those were judged by our annotators as not having the same meaning. % For example former White House chief of staff Mark Meadows was born in an army base in France, but he would not describe himself as ``from'' France.

Below is an example of a precision error: 

\vspace{1em}
\hspace{-1em}\begin{tabular}{@{}|p{0.94\columnwidth}|@{}}
    \hline
    \textbf{Input:} \small\texttt{Zaoyang | isPartOf | Hubei} \\
    \small\texttt{Nie\_Haisheng | mission | Shenzhou\_6} \\
    \small\texttt{Nie\_Haisheng | birthPlace | Zaoyang} \\
    \hline
    \textbf{Target:} \\Born in Zaoyang city, Hubei, Nie Haisheng participated in the Shenzhou 6 mission.\\
    \hline
    \textbf{Implied:} \\
    \small\texttt{Nie\_Haisheng | birthPlace | Hubei} \\
    \hline
\end{tabular}
\vspace{1em}

In the example, {\footnotesize\texttt{Nie\_Haisheng | birthPlace | Zaoyang}} and {\small\texttt{Zaoyang | isPartOf | Hubei}} together imply {\small\texttt{Nie\_Haisheng | birthPlace | Hubeia}} and the SP picked up on this by generating the implied relation.  This was accepted by our annotators, and our metrics show it as a precision loss -- the generated text includes a triple that was not in the desired parse.\footnote{It may be possible in theory to enumerate implied relations by writing rules to avoid penalizing the text presented to the raters for including the semantics implied by the desired triples. However, this would make results more difficult to reproduce, and instead note that this is a shortcoming of the evaluation of the generated semantics.}
